Contextual Recommendations and Low-Regret Cutting-Plane Algorithms

We consider the following variant of contextual linear bandits motivated by routing applications in navigational engines and recommendation systems. We wish to learn a hidden $d$-dimensional value $w^*$. Every round, we are presented with a subset $\mathcal{X}_t \subseteq \mathbb{R}^d$ of possible actions. If we choose (i.e. recommend to the user) action $x_t$, we obtain utility $\langle x_t, w^* \rangle$ but only learn the identity of the best action $\arg\max_{x \in \mathcal{X}_t} \langle x, w^* \rangle$. We design algorithms for this problem which achieve regret $O(d\log T)$ and $\exp(O(d \log d))$. To accomplish this, we design novel cutting-plane algorithms with low "regret" -- the total distance between the true point $w^*$ and the hyperplanes the separation oracle returns. We also consider the variant where we are allowed to provide a list of several recommendations. In this variant, we give an algorithm with $O(d^2 \log d)$ regret and list size $\mathrm{poly}(d)$. Finally, we construct nearly tight algorithms for a weaker variant of this problem where the learner only learns the identity of an action that is better than the recommendation. Our results rely on new algorithmic techniques in convex geometry (including a variant of Steiner's formula for the centroid of a convex set) which may be of independent interest.

==> contextual-recomendation.tex <==
\section{List Contextual Recomendation} \label{sec:contextual-recomendation}
In this section, we consider the problem where we are allowed to offer a list of possible actions
$L_t \subseteq \X_t$ and we measure regret against the best action in the list:
\[ \loss_t =  \bkt{w^*}{x_t^* } - \max_{x \in L_t} \bkt{w^*}{x}.\] 
Our main result is that if the list is allowed to be of size $O(d^4)$ then it is possible to achieve total regret $O(d^2 \log d)$.

The recommended list of actions will be computed as follows: given the knowledge set $K_t$, let $D$ be the discretization of the curvature path with parameter $k = 200 d^4$ obtained in Lemma \ref{lem:curve-discretization}. Then for each $p_i \in D$ find an arbitrary $x_i \in \BR(p_i) := \argmax_{x \in \X_t} \bkt{p_i}{x} $ and let $L_t = \{x_1, x_2, \hdots, x_k\}$.

\begin{theorem} \label{thm:low-regret-list}
There exists an algorithm which plays the list $L_t$ defined above suffers a total regret that is at most $O(d^2 \log d) $. 
\end{theorem}
\begin{proof}

The overall structure of the proof will be as follows: we will show that for each integer $j \geq 0$, the algorithm can incur loss  between $100d \cdot 2^{-j}$ and  $200d \cdot 2^{-j}$ at most $O(jd)$ times. Hence the total loss of the algorithm can be bounded by $\sum_{j=1}^\infty O(jd) \cdot 2^{-j} d \leq O(d^2 \log d)$.\\

\emph{Potential function:} This will be done via a potential function argument. As usual, we will keep track of knowledge $K_t$ which corresponds to all possible values of $w$ that are consistent with the observations seen so far. $K_1 = \B$ and:
$$K_{t+1} = K_t \cap \left[\cap_{i \in L_t} \{w \in \R^d; \bkt{x^* - x}{w} \geq 0\} \right]$$
Associated with $K_t$ we will keep track of a family of potential functions:
$$\Phi_t^j = \Vol(K_t +  2^{-j} \B)$$
Since $K_1 \supseteq K_2  \supseteq K_3  \supseteq ...$ the potentials will be non-increasing: $\Phi_1^j \geq \Phi_2^j \geq \Phi_3^j \geq ...$. One other important property is that the potential functions are lower bounded:
\begin{equation}\label{eq:potential_lower_bound}
\Phi_j^t \geq \Vol(2^{-j}\B) = 2^{-jd} \Vol(\B)
\end{equation}
We will argue that if we can bound the loss at any given step $t$ by $200 2^{-j}d$, then $\Phi^j_{t+1} \leq 0.9 \cdot \Phi^j_t$. Because of the lower bound in equation \ref{eq:potential_lower_bound}, this can happen at most $$O\left(\log\left(\frac{\Phi_j^1 }{ 2^{-jd} \Vol(B)}\right)\right) = O\left(\log\left(\frac{(1+2^{-j})^d\Vol(\B)}{ 2^{-jd} \Vol(B)}\right)\right) \leq O(jd)$$

\emph{Bounding the loss:} We start by bounding the loss and depending on the loss we will show a constant decrease in a corresponding potential function. Let
$$x^*\in \argmax_{x \in \X_t} \bkt{w^*}{x}$$
If $x^*$ is in the convex hull of $L_t$ then there must some of the points in $x_i \in L_t$ that is also optimal, in which case the algorithm incurs zero loss in this round and we can ignore it. Otherwise, we can assume that $x^*$ is not in the convex hull of $L_t$.

In that case, define for each $x_i \in L_t$ the vector:
$$v_i = \frac{x^* - x_i}{\norm{x^*-x_i}_2}$$
Consider the index $i$ that minimizes $\width(K; v_i)$ and use this point to bound the loss:
$$\begin{aligned}
\loss_t & = \min_{x \in L_t} \bkt{w^*}{x^*-x} \leq \bkt{w^*}{x^*-x_i} \leq \bkt{w^* - p_i}{x^* - x_i}  \\ & = \bkt{w^* - p_i}{v_i} \cdot \norm{x^* - x_i}  \leq 2\bkt{w^* -p_i}{v_i} \leq 2 \width(K, v_i)
\end{aligned}$$
The second inequality above follows from the definition of $x_i$ since $x_i \in \argmax_{x \in \X_t} \bkt{p_i}{x}$ it follows that $\bkt{p_i}{x_i - x^*} \geq 0$.\\

\emph{Charging the loss to the potential} We will now charge this loss to the potential. For that we first define an index $j$ such that:
$$j = - \left\lceil \frac{\width(K,v_i)}{100 d} \right\rceil$$
With this definition we have:
$$\loss_t \leq 2 \width(K,v_i) \leq 200 d 2^{-j}$$
Our final step is to show that the potential $\Phi_t^j$ decreases by a constant factor. For that we will use a combination of the discretization in Theorem \ref{lem:curve-discretization} and the volume reduction guarantee in Lemma \ref{lem:volume-reduction}.

First consider the point:
$$g_i = \cg(K + 2^{-j} \B)$$
Since it is on the curvature path, there is a discretized point $p_\ell \in D$ such that:
$$\vert \bkt{v_\ell}{g_i - p_\ell} \vert \leq \width(K, v_\ell)/(50 d)$$
Together with the facts that $\bkt{w^*}{v_\ell} \geq 0$ and $\bkt{p_\ell}{v_\ell} \leq 0$ we obtain that:
$$\bkt{w^* - g_i}{v_\ell} = \bkt{w^* - p_\ell}{v_\ell} + \bkt{ p_\ell - g_i}{v_\ell} \geq -\width(K, v_\ell)/(50d)$$
This in particular implies that:
$$K_{t+1} \subseteq \tilde{K}_{t+1} := K_t \cap \{w \in \R^d; \bkt{w - g_i}{v_\ell} \geq  -\width(K, v_\ell)/(50d)\}$$
We are now in the position of applying \Cref{lem:volume-reduction} with $r = 2^{-j}$. Note that $$r = 2^{-j} \leq \frac{ \width(K, v_i)}{50 d} \leq \frac{\width(K, v_\ell)}{50 d}$$
where the last inequality follows from the choice of the index $i$ as the one minimizing $\width(K, v_i)$. Applying the Theorem, we obtain that:
$$\Vol(K_{t+1} + 2^{-j}\B) \leq \Vol(\tilde{K}_{t+1} + 2^{-j}\B) \leq 0.9 \cdot \Vol(K_t + 2^{-j}\B)$$
which is the desired decrease in the $\Phi^j_t$ potential. This concludes the proof.
\end{proof}


